A Unified Benchmark for Aerial-Enhanced Autonomous Driving: The KITScenes Aerial Dataset

Aerial imagery provides complementary spatial context for autonomous driving by exposing road structure beyond the immediate perception range of onboard sensors. Yet map construction from aerial imagery, aerial-assisted online HD mapping, and cross-view localization are typically studied on separate data and benchmarks. We introduce KITScenes Aerial, an extension of the KITScenes Multimodal dataset that augments synchronized onboard sensor data, vehicle poses, and rich Lanelet2 map annotations with spatially associated aerial imagery and higher-resolution neural representations, providing a common basis for a variety of research tasks. Our mapping evaluation focuses on all 53 KITScenes map classes across different model designs, spatial ranges, and aerial resolutions, while retaining compatibility with the widely used three-class setting. Representative baselines show that aerial context is particularly beneficial for fine-grained and extended-range mapping, more than doubling 53-class mAP at the larger mapping extent. Higher-resolution aerial imagery yields a further 4.3 mAP (+24 %) improvement, with gains extending to challenging map elements such as traffic lights. We additionally evaluate cross-view localization under geographically disjoint conditions, where an adapted fine-grained feature-matching baseline achieves a mean translation error of 5.13 m. KITScenes Aerial thus enables unified study of aerial and ground-level information across complementary mapping and localization tasks. Project page: https://kitscenes.com/aerial

==> sec/tables_figures/tableset2_defs.tex <==
\makeatletter

\@ifundefined{hbfull}{%
  \@ifundefined{tikz}{%
    \DeclareRobustCommand{\hbfull}{\ensuremath{\bullet}}%
    \DeclareRobustCommand{\hbhalf}{\ensuremath{\odot}}%
  }{%
    \newsavebox{\hb@fullbox}%
    \newsavebox{\hb@halfbox}%
    \sbox{\hb@fullbox}{\tikz[baseline=-0.55ex]{\fill (0,0) circle (0.52ex);}}%
    \sbox{\hb@halfbox}{%
      \tikz[baseline=-0.55ex]{%
        \begin{scope}
          \clip (0,-0.6ex) rectangle (0.6ex,0.6ex);
          \fill (0,0) circle (0.52ex);
        \end{scope}
        \draw[line width=0.16ex] (0,0) circle (0.52ex);}}%
    \DeclareRobustCommand{\hbfull}{\usebox{\hb@fullbox}}%
    \DeclareRobustCommand{\hbhalf}{\usebox{\hb@halfbox}}%
  }%
}{}

\@ifundefined{nosup}{\DeclareRobustCommand{\nosup}{--}}{}
\@ifundefined{unk}{\DeclareRobustCommand{\unk}{\textbf{?}}}{}
\@ifundefined{nrep}{\DeclareRobustCommand{\nrep}{\textit{n/r}}}{}
\@ifundefined{sups}{\DeclareRobustCommand{\sups}[1]{\textsuperscript{#1}}}{}
\providecommand{\cmarkbracketsup}[1]{\llap{(}\checkmark\rlap{)\textsuperscript{#1}}}

\@ifundefined{kitrow}{%
  \definecolor{kitshade}{rgb}{0.925,0.945,0.972}%
  \@ifundefined{rowcolor}{\newcommand{\kitrow}{}}%
                         {\newcommand{\kitrow}{\rowcolor{kitshade}}}%
}{}

\makeatother

